AI-based Attacker Models for Enhancing Multi-Stage Cyberattack Simulations in Smart Grids Using Co-Simulation Environments

The transition to smart grids has increased the vulnerability of electrical power systems to advanced cyber threats. To safeguard these systems, comprehensive security measures-including preventive, detective, and reactive strategies-are necessary. As part of the critical infrastructure, securing these systems is a major research focus, particularly against cyberattacks. Many methods are developed to detect anomalies and intrusions and assess the damage potential of attacks. However, these methods require large amounts of data, which are often limited or private due to security concerns. We propose a co-simulation framework that employs an autonomous agent to execute modular cyberattacks within a configurable environment, enabling reproducible and adaptable data generation. The impact of virtual attacks is compared to those in a physical lab targeting real smart grids. We also investigate the use of large language models for automating attack generation, though current models on consumer hardware are unreliable. Our approach offers a flexible, versatile source for data generation, aiding in faster prototyping and reducing development resources and time.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> chapter1.tex <==
%-- A nomenclature section should be added to help the reader understand and follow better the variables used throughout the paper.
%-- The introduction section could be divided into: a) Motivation and Background; b) Relevant Literature; c) Contributions and Organization. Clearly state what is new in this study compared to earlier studies.
%-- The legibility of figures should be increased; please provide high-resolution figures.
%-- The recommended minimum and maximum number of references is 15 and 25, respectively. Also, the majority of references should be up-to-date (less than 3 years old).
%-- Finally, please make sure that the paper is written in clear and understandable English language. Proofreading by a native speaker is always advisable.
%
\section{Introduction}\label{sec:intro}

As power grids increasingly incorporate \ac{ICT}, they become more interconnected with external devices, removing the natural barrier of isolation and exposing them to new cybersecurity threats. A notable example is the 2015 Ukraine cyberattack, which resulted in a significant blackout. Cybersecurity in power systems is a vital, ongoing process based on prevention, detection, and reaction, guided by standards such as IEC 62351 and IEC 62443. Additionally, improving cybersecurity resilience and protecting critical infrastructures are emphasized legally with emerging regulations like NIS2.

Security shortcomings, which combine a lot of software that may include vulnerabilities and even the used protocols like IEC 104, commonly used in SCADA systems, which lack authentication and encryption. Implementing security enhancements, including evaluating new metrics, analyzing component behavior in a network, examining logs, and running \acp{IDS} in smart grids.  These steps are promising but all depend on data or reference values for analysis. While some openly accessible datasets exist, many are either poorly maintained, too specific, or have other shortcomings.

Grid operators tend to keep their data private due to security concerns, forcing researchers to either build their own laboratories or simulate smart grids themselves. Modelling smart grids in a laboratory requires expertise, time to install hardware, and significant expense to operate. Implementing and setting up even a small laboratory demands professionals from various domains.

Several studies use co-simulation environments to assess advanced network configurations and security measures with real hardware components. Johnson et al. [JOH20] developed the SCEPTRE tools, combining simulated components with physical inverters in a hardware-in-loop (HIL) approach to test performance and resilience against cyberattacks. However, these attacks had to be performed manually, making the approach hard to maintain and scale with the growing number of attack methods.

Arguello et al. [ARG19] estimated worst-case scenarios using parametric emulation and analytical approximations, searching for the largest impact a cyberattack could have on a power grid. Although loads were simulated, communication between components was limited, failing to represent the steps of an attack effectively. Other studies evaluated multiple attack methods through simulations with and without cyberattacks [LE19]. Some tools could generate reports and run simple distributed denial of service (DDoS) attacks, while others focused solely on co-simulation. Manual attacks simulated the effects by increasing virtual network delay or replacing control values, but did not model how an attacker achieves these manipulations.

Manual red teaming approaches face challenges in consistency and scalability, making automation a promising solution. Frameworks like Plan2Defend [CHO21] and autonomous agents for cyber defense [VYA23] use autonomous methods to mitigate ongoing cyberattacks or execute plans, reducing response time. While these methods evaluate system security and monitor activity, they lack the ability to generate attack data, relying on manual implementation of sophisticated attacks for training.

Proactive testing via attack emulation allows for hardening security before actual attacks occur. Although individual cyberattacks on smart grids have been analyzed, there is less focus on general frameworks for complex data generation. Intrusion detection systems (IDSs) require extensive data to evaluate performance and adapt to varying network topologies.

Our method builds on the works of Bleser and Kehrein [BLE23], [KEH21]. Bleser demonstrated creating a digital twin of smart grids in a co-simulation environment, replicating laboratory equipment and topology realistically. Kehrein's approach generates attack scenarios based on real-world attacks in a more autonomous and dynamic manner. Configuring and simulating scenarios in our co-simulation allows for fast generation of network logs for further evaluation.

To address these challenges, we propose a method for automatically running cyberattacks inside a simulation environment, generating network logs and power simulation results. This approach allows for the creation of datasets for configurable network topologies and various attack scenarios, improving data availability and eliminating the need for expensive setups. Combining these works, our method generates data from a broad range of attack scenarios, simulated realistically in a co-simulation environment, providing data applicable to laboratory-like grid architectures. This comprehensive approach enables the extraction of valuable data, facilitating the study and enhancement of smart grid cybersecurity. Our contributions are the following:

\begin{itemize}
\item Definition of the problem and corresponding requirements for our method, and deduction of a general concept for our work.
\item Design and assessment of the AI-based attacker model in a simulation environment, detailing the physical laboratory and co-simulation structure, the autonomous agent's operation, deployment environments, and the data generation process.
\item Evaluation of the data generation process via comparative analysis with a physical laboratory using a digital twin approach.
\end{itemize}

==> chapter2.tex <==
\section{Background}\label{sec:background}
\subsection{Smart Grid Control Architecture} \label{subsec:background_smartgrid}
Compared to early power grids that directly connected energy generators with consumers, modern energy infrastructure is much more complex. The increasing use of energy sources such as photovoltaic (PV) systems and wind turbines makes regulation and coordination more challenging. When these generators are distributed and connected to a large power grid without bundling their loads in a large converter, special regulation and balancing are required before their energy can be fed into the grid. Smart grids provide a solution as cyber-physical systems that connect energy sources with consumers and enable communication between actors to balance and control the power grid reliably.

\begin{figure}[htbp]
    \centerline{\includegraphics[width=\columnwidth]{figures/Purdue.pdf}}
    \caption{Purdue reference model for smart grids}
    \label{fig:purdue_model}
\end{figure}

Understanding smart grid operation requires knowledge of its components:

\begin{itemize}
    \item \textbf{Terminal Units}: Responsible for communication within smart grids, these units collect and transmit data and send and receive control commands for connected actuators and sensors. They are divided into remote terminal units (RTUs), which connect to physical equipment, and master terminal units (MTUs), which aggregate data from RTUs.

    \item \textbf{Supervisory Control and Data Acquisition (SCADA) Systems}: These systems handle data reported by terminal units, processing it to deduce necessary commands for adjusting grid behavior. They provide human-machine interfaces (HMIs) for users to visualize data and control grid components remotely.

    \item \textbf{Intelligent Electronic Devices (IEDs)}: These controllers, integrated into power equipment, collect data from sensors and issue commands to the equipment. They communicate directly with SCADA systems or via RTUs.

    \item \textbf{Decentralized Energy Resources (DERs)}: Small components that either supply or demand electricity. They can connect directly to the grid or be aggregated to feed their load into the grid. Examples include microturbines, solar arrays, and energy storage systems.

    \item \textbf{Protocols}: Essential for data exchange in smart grids, common protocols include IEC 60870-5-104 (IEC 104) and Modbus, both of which work over TCP/IP networks to connect SCADA systems with terminal units. Despite their importance, these protocols lack integrated security concepts and are vulnerable to various cyberattacks. Secure Shell (SSH) is another important protocol used for remote access, posing potential security threats if authorization is compromised.
\end{itemize}

The overall structure of an industrial control system (ICS) can be described using the Purdue model, proposed by Williams et al. in the 1990s.  This model segments the network into multiple layers, allowing separation between operational technology (OT) and information technology (IT) systems. The model defines a hierarchy for communication between layers, ranging from external services at the highest level (Level 5) to the actual control of physical actors at the lowest level (Level 0).

The layers of the Purdue model are as follows:

\begin{itemize}
    \item \textbf{Level 5 (Enterprise Zone)}: Contains general IT systems accessible to external clients, offering the most open services.
    \item \textbf{Level 4}: Focuses on data and software for production scheduling and operational management, including mail servers and other broadly accessible services.
    \item \textbf{Demilitarized Zone (DMZ)}: Separates IT and OT systems, using firewalls to block most communication protocols, securing sensitive data by preventing outgoing communication.
    \item \textbf{Level 3 (Manufacturing Zone)}: The highest level in the OT site, containing local workstations and data collections for process data.
    \item \textbf{Level 2}: Houses area control systems that collect and monitor data within subsystems.
    \item \textbf{Level 1}: Consists of controlling elements that send measured values to data collectors and control physical actors and sensors.
    \item \textbf{Level 0}: Includes all machinery performing physical tasks and measurements.
\end{itemize}

Despite being proposed decades ago, the Purdue model remains widely applied, particularly in the context of cybersecurity for cyber-physical systems.

\subsection{Simulation Aspect} \label{subsec:background_simulation}

To simulate smart grids, we must understand what simulation entails and how it can be achieved. Generally, simulation involves imitating real-world systems via software. Instead of creating a single, complex model, it's more efficient to implement smaller components separately and combine them to model complex systems. These components can run in individual virtual environments to prevent interference.

Virtualization involves running individual processes or entire operating systems (OSs) on multiple virtual computers, each using a portion of the host computer's resources. 
In contrast to the well-established approach of bundling and isolating software in virtual machines (VMs), we implemented our work with the help of containerization. While VMs include their own OS, containerization allows the software to share the resources with the host they are run on dynamically, making them more efficient to run in parallel. These instances are called containers and are built according to a blueprint, that defines the corresponding software, memory and network available when instantiating it. Containers can communicate through virtual network, sending actual network packets between specific instances.

%\begin{itemize}
%    \item \textbf{Virtual Machines (VMs)}: These are well-established methods for isolating software and its dependencies into a bundle that runs as a separate execution environment. VMs contain their own OS, running parallel to the host system, ensuring isolation. However, this isolation comes with higher memory usage.
%    \item \textbf{Containerization}: This more recent tool distributes software by creating self-contained environments using images that serve as blueprints for the software, memory, and networking configurations. Containers share the host's OS, making them more resource-efficient than VMs. Containers and VMs can communicate through virtual networks, sending actual network packets between specific instances. 
%\end{itemize}



Virtual networks allow communication between specific containers or VMs, creating separated networks on the same host. Orchestration tools further streamline the setup by reading configuration files to define containers and their settings, automating their deployment and management. 

Using container orchestration, we can automate the deployment of pre-configured containers and their virtual networks. This enables running complex scenarios with shared computing resources, making large-scale simulations less resource-demanding.

A key goal of our work is to run simulations automatically and incorporate systems classified as artificial intelligence (AI). 

\begin{itemize}
    \item \textbf{Automation}: In software, automation refers to the automatic operation of software with minimal user interaction. A program executing pre-defined tasks is considered automatic.
    \item \textbf{Autonomy}: When a program makes decisions and reacts to its environment, it is considered autonomous. According to Formosa et al., autonomy is a spectrum: the more parameters a system considers when making decisions, the more autonomous it acts.
\end{itemize}

The European Commission's Artificial Intelligence Act defines AI systems as machine-based systems designed to operate with varying levels of autonomy. These systems may exhibit adaptiveness and generate outputs such as predictions, content, recommendations, or decisions that influence environments.

\subsection{Cybersecurity in Smart Grids} \label{subsec:background_cybersecurity}
As smart grids increasingly resemble traditional computer networks, they become susceptible to similar cyberattacks \cite{li2012}. Below are some prevalent attack schemes and their potential combinations for more complex routines.

\begin{itemize}
    \item \textbf{Reconnaissance:} This involves gathering information about the target, such as scanning for services, phishing for information, and researching networks and organizational structures. This step is crucial as it informs attackers where and how to strike.
    
    \item \textbf{Initial Access:} This is the first infiltration that grants the attacker entry to the system, achieved through physical access, phishing, or credential theft. It provides a foothold for further exploits.
    
    \item \textbf{Execution:} Techniques in this category start new processes or manipulate existing ones to run the attacker's code. This can be done through phishing, software manipulation, or credential use to execute commands.
    
    \item \textbf{Persistence:} Ensuring long-term access, attackers might create new user accounts, schedule periodic jobs, or manipulate software to run their code. Persistent attacks allow data collection over time or enable future exploits, such as Distributed Denial of Service (DDoS) attacks.
    
    \item \textbf{Command-and-Control (C2):} These techniques enable communication between the attacker and compromised hosts. Attackers use normal network traffic to create covert communication channels for issuing new commands.
    
    \item \textbf{Exfiltration and Impact:} These final stages often cause significant damage, such as sending sensitive data to the attacker or rendering services unavailable through Denial of Service (DoS) attacks. These techniques are often the ultimate goal of an attack.
\end{itemize}

Attackers often combine techniques from different categories to execute complex attacks, making them harder to detect and defend against.

Advanced Persistent Threats (APTs) involve multiple stages executed sequentially. These stages typically include reconnaissance, initial access, persistence, and command-and-control, followed by the final impact. The complexity of APTs, with their numerous specialized steps, targets specific victims over a prolonged period, making them difficult to track and defend against.

For instance, the DARPA 2000 dataset features various DDoS attacks comprising multiple steps \cite{ahm2016}. A simpler attack might include IP address scanning, service exploitation, and a subsequent DDoS attack using compromised hosts. A more sophisticated attack, such as island-hopping, spreads malware through infected PDFs sent across the network until a desired database service is found. These examples highlight how combining different attack methods and exploiting vulnerabilities can allow attackers to gather extensive information and manipulate network components.

%For instance, the DARPA 2000 dataset features various DDoS attacks comprising multiple steps \cite{ahm2016}. Simple attacks might use sequential network scans followed by a DDoS attack, whereas more sophisticated attacks, such as island-hopping, could distribute malware via malicious PDFs sent across the network until a specific target is found. These examples highlight how combining different attack methods and exploiting vulnerabilities can allow attackers to gather extensive information and manipulate network components.

To defend against these attacks, it is essential to implement comprehensive cybersecurity strategies, including:
\begin{itemize}
    \item \textbf{Network Security:} Employ firewalls, intrusion detection systems (IDS), and intrusion prevention systems (IPS) to monitor and control incoming and outgoing network traffic based on predetermined security rules.
    
    \item \textbf{Access Controls:} Enforce strong authentication mechanisms and limit user permissions to minimize the risk of unauthorized access.
    
    \item \textbf{Regular Updates and Patching:} Keep systems and software updated to protect against known vulnerabilities.
    
    \item \textbf{Employee Training:} Educate employees about phishing and other social engineering techniques to reduce the likelihood of successful attacks.
    
    \item \textbf{Incident Response Plans:} Develop and regularly update incident response plans to quickly address and mitigate the impact of cyber incidents.
\end{itemize}

==> chapter3.tex <==
\section{Methodology}\label{sec:method}
\subsection{Requirement} \label{subsec:method_req}

We aim to create a framework for generating network logs of smart grids during multi-stage cyberattacks. The current lack of available data for network logs of intrusions and the potential of co-simulations as a new data source necessitates ensuring the quality of synthetic network logs. A reproducible method to create these logs is essential for systematically comparing different impacts without the need for expensive equipment or a complete laboratory setup. A method making cyberattacks easily reproducible and configurable would facilitate consistent data analysis and generate high-quality, otherwise scarce data.

\begin{itemize}
    \item \textbf{Virtual Smart Grid Simulation:} To generate log data, we need a simulation that resembles real grids, incorporating the basic components common to real-world smart grids. This simulation should be entirely virtual to eliminate specific hardware demands.
    
    \item \textbf{Recordable Network Communication:} The simulation must log network traffic, capturing packet data on the transport layer.

    \item \textbf{Integrated Attack Simulation:} We need to capture anomalies during adversary actions within the simulation to utilize the network and the simulation's components' logic effectively.
\end{itemize}

\begin{itemize}
    \item \textbf{Realistic Impact on Data Output:} The data generated must be usable like those measured on real hardware, accurately capturing the impact of cyberattacks.

    \item \textbf{Configuration-Based Setup:} The simulation should be configurable to cover various scenarios and topologies, allowing automatic setup based on user-defined parameters to ensure scalability and prevent initialization errors.

    \item \textbf{Autonomous Attacks with Modular Methods:} The simulation should support multiple attack methods, handling multi-stage attacks autonomously. This ensures reproducibility of complex attacks and allows the selection of the best-suited methods.

    \item \textbf{Automatic Data Export:} The simulation should yield all relevant data and logs automatically, ensuring consistency and reproducibility across different scenarios and runs.

    \item \textbf{Offline Availability:} The simulation should operate without internet access, adhering to the segmented network architecture typical in smart grids.

    \item \textbf{Clean and Consistent Network Logs:} The generated network traffic should maintain uniformity to minimize fluctuations across different runs, ensuring the impact of attacks is clear.
\end{itemize}

For our data, two main properties are crucial: realism and consistency across different scenarios. Realistic data must closely depict the individual nuances of each attack, and consistency ensures that data output is structured similarly across different runs. We identified four main metrics to analyze each attack scenario:

\begin{itemize}
    \item \textbf{Power Simulation Results:} The simulation must handle the effects on power generation and distribution accurately, reflecting any changes in component behavior due to cyberattacks.

    \item \textbf{Protocol Distribution:} This metric examines the distribution of communication across different protocols during an attack. Stability in protocol usage indicates consistent behavior of the involved components.

    \item \textbf{Timely Spread:} The same attack should be executed within a similar timeframe, with the attacker performing tasks at consistent points during the simulation.

    \item \textbf{Traffic Volume:} This focuses on the amount of data communicated in the network. Consistency in traffic volume and direction among different components during attacks indicates reliable simulation behavior.
\end{itemize}

These metrics help ensure that the generated data is both realistic and consistent, providing a robust foundation for analyzing and improving smart grid cybersecurity. Our methodology focuses on these requirements, and we will evaluate how these were satisfied by our framework at the end of this work.

\subsection{Design Idea} \label{subsec:method_deisgn}

To meet the requirements for generating realistic network logs of smart grids during multi-stage cyberattacks, we propose a design that ensures realistic simulation, modularity, and scalability without compromise.

Each component in the simulation must mimic its physical counterpart's behavior. This includes modeling interactions with other elements in the simulation environment, especially data exchanges and remote control messages, to produce realistic data.

A modular structure allows flexible configuration of scenarios using reusable components. Containerization tools, such as Docker, support this modularity. Using Docker images for the smart grid actors enables easy instantiation of multiple components with the same logic but different parameters. Networking configurations ensure that only selected connections are enabled between containers, specifying maximum bandwidth and simulated latency to create realistic network logs, even on a single host. Users can define the topology in readable configuration files, adapting it as needed.

Orchestration tools help manage complex network topologies and prevent user errors. These tools can derive a whole simulation scenario from a single file, handling initialization and setup. Established orchestration tools also support scripts triggered after containers start or stop, facilitating the setup and extraction of network logs.

The attacks run in the simulation should be modular and not handcrafted specifically for one scenario.
By integrating existing attack methods based on real-world cyberattacks, we ensure the framework's flexibility and reduce the need for specialized cybersecurity expertise.

With these design choices, we chose a Docker-based approach leveraging containerization capabilities. Using a collection of pre-existing components for network communication and power simulation, we adopted the co-simulation environment proposed in \cite{VEL21}.

This approach employs several tools and frameworks that align with our design decisions:

\begin{itemize}
    \item \textbf{rettij}: Utilizes Kubernetes orchestration, allowing the use of configuration files to define components and network connections in virtual smart grids via Docker images.
    \item \textbf{Mosaik and Panda Power}: Add power simulation capabilities, enabling realistic power grid simulations \cite{THU18}.
\end{itemize}

Based on this co-simulation environment, we developed an attacker container that autonomously performs specified cyberattacks. This attacker integrates seamlessly into the co-simulation, generating network logs and power simulation results applicable to real-world scenarios.

By combining these components, our framework facilitates the generation of realistic, consistent, and high-quality data for analyzing and improving smart grid cybersecurity.


\section{Approach}\label{sec:approach}
\subsection{Co-Simulation Environment} \label{subsec:approach_cosim}

Our work utilizes the co-simulation software Mosaik, which groups individual simulators in a common context to build scenarios modularly \cite{OFE22}. Each simulator provides the functionality of real-world components, enabling the reconstruction of existing physical scenarios and the reuse of logic across varying simulator combinations.

To simulate the power grid and communication within a laboratory setup, we use Panda Power and other network communication simulators within Mosaik. Panda Power discretely simulates loads at each time step, while network communication simulators manage the interactions between components. Mosaik synchronizes these simulators, iterating through each simulation step and ensuring timely execution based on the current simulation time.

Mosaik connects modular simulators, synchronizing their communication to create a discrete environment. It iterates through each simulation step, checking if enough time has passed to execute the next step and then instructs the corresponding simulator to proceed.

Panda Power generates measurements for the virtual power grid, simulating components based on a predefined configuration file. This file describes power generators, transformers, buses, and power lines. The framework extracts detailed information about current usages and loads across all components \cite{THU18}.

Terminal unit nodes handle IEC 104 communication, running as either RTUs or MTUs. They connect to a Mosaik server, translating measurements and commands to Panda Power to update the simulation. Terminal units can be configured to use predefined values or send specific commands at designated times.

Rettij initializes virtual networks and starts containers, simplifying network connection definitions. The topology configuration specifies the components and their respective images. Rettij also handles virtual delays and bandwidth limitations, simulating realistic network conditions for larger grids.

We use a switch developed by the rettij team to create a virtual network, connecting all relevant components. The switch handles packet forwarding, with packet capturing initiated and stopped via rettij commands. This setup ensures comprehensive network logs with correctly ordered packets. The virtual network separates the communication of terminal units from Mosaik and Panda Power servers, keeping their messages out of the switch logs.

Managing networking between containers is a key challenge. The network must be segmented, with components communicating only with selected others. Rettij allows defining network topology in YAML format, modeling LAN connections within the laboratory.

\begin{figure}[htbp]
     \centerline{\includegraphics[width=\columnwidth]{figures/CoSim.pdf}}
    \caption{Topology inside the co-simulation. All components are realized by individual containers. The virtual network emulates local laboratory communication, with only traffic through the switch considered in the network logs.}
    \label{fig:topology}
\end{figure}

%We decided on a Docker-based approach leveraging containerization capabilities. Using pre-existing components for network communication and power simulation, we adopted the co-simulation environment proposed in \cite{VEL21}. This setup includes Mosaik and Panda Power, enhancing power simulation capabilities \cite{THU18}.

The rettij framework uses Kubernetes orchestration, defining components and network connections in virtual smart grids via Docker images. The combination of Mosaik, Panda Power, and rettij provides a robust environment for simulating and analyzing cyberattacks on smart grids.

By integrating modular attacks based on real-world cyberattacks, we ensure flexibility and reduce the need for specialized cybersecurity expertise. Our attacker container autonomously performs specified cyberattacks within the co-simulation, generating realistic and high-quality network logs and power simulation results.

\subsection{Attack Emulation} \label{subsec:approach_emulation}

To complete our scenarios, we need to integrate attacking logic into our simulation environment, leveraging rettij’s ability to define timed script execution. This section outlines our approach using MITRE Caldera™, a step-based attack emulation tool that aligns well with our co-simulation needs due to its structured and workflow-oriented nature. Caldera employs a central command-and-control (C2) server with planning algorithms to manage attack steps, facilitating iterative execution of multi-stage attacks within Mosaik.

Several alternatives exist for attack emulation, but each has limitations compared to Caldera:

\begin{itemize}
    \item \textbf{Atomic Red Team}: A collection of scripts for testing ATT\&CK-defined attack schemes, including platform-specific code for Windows. However, our environment uses Linux containers, making this less relevant.
    \item \textbf{Splunk}: A proprietary platform for IT security testing, visualization, and management. Its closed-source nature complicates integration with Mosaik.
    \item \textbf{MulVal}: Assesses network security based on vulnerability reports but does not emulate attacks directly.
\end{itemize}

We chose Caldera due to its autonomous execution, active development, extensibility via plugins, and customizable Python scripts.


Caldera's attack execution relies on several key components:


Abilities are YAML-defined scripts and commands that implement ATT\&CK techniques. Each ability is identified by a unique ID and includes executors specifying the platform and command to be run, such as Shell for Linux. Abilities may include payloads downloaded as needed and cleanup commands to minimize traces on victim machines. For example, an ability to capture network traffic might look like this:

\begin{verbatim}
name: Capture Network Traffic (TCPDump with Scapy)
id: 1b27e1f8-af08-47eb-b3dc-100c1d697413
platform: linux
command: /bin/python tcpdump.py -t 150
cleanup: [/bin/rm tcpdump.py]
payloads: [tcpdump.py]
\end{verbatim}


Adversaries are constructs combining multiple abilities to form multi-stage attack plans. Each adversary definition ensures that abilities are executed in sequence, with dependencies checked for each step. For example, an adversary performing a Denial of Service (DoS) attack might include abilities for network scanning, host enumeration, and attack execution.


Fact sources store and manage data used across agents and abilities, allowing for dynamic execution based on collected or pre-defined information. Facts are labeled values, such as IP addresses or credentials, that can trigger abilities. Rules filter which facts are used, ensuring targeted execution. For instance:

\begin{verbatim}
name: restrictions
facts:
  - trait: host.local.ip
    value: 10.1.2.*
  - trait: host.local.ip
    action: DENY
    match: 10.42.*
\end{verbatim}

Operations combine adversaries and fact sources, specifying execution details such as agent groups, step intervals, and execution mode (automatic or manual). Operations control the overall attack flow, leveraging modular definitions to reuse attack logic and necessary information.


To execute an attack, we follow these steps:

\begin{enumerate}
    \item \textbf{Start the C2 Server}: The C2 server orchestrates components, provides payload access, and listens for agent connections. It runs locally without internet access, maintaining all necessary attack information.
    \item \textbf{Connect an Agent}: An agent, a client executable on a compromised machine, connects to the C2 server. It communicates via HTTP packets, providing minimal obfuscation. Agents are categorized by group identifiers for targeted attack execution.
    \item \textbf{Execute an Operation}: We select the agent group and adversary for execution. The operation uses Caldera’s planning module to determine and send instructions to agents based on available facts and adversary requirements. Agents execute commands, collect outputs, and send results back to the server for parsing and further execution.
    \item \textbf{Cleanup}: To minimize traces, agents execute cleanup commands either remotely by the server or as part of adversary completion.
\end{enumerate}

This structured approach ensures detailed control and parallel execution across multiple agents, enhancing the robustness of our attack emulation within the simulated smart grid environment. The execution flow is illustrated in Figure~\ref{fig:execution-flow}, highlighting the seamless integration of Caldera’s components to perform sophisticated cyberattack simulations.

\begin{figure}[htbp]
\centerline{\includegraphics[width=.8\columnwidth]{figures/sequence_c2.pdf}}
\caption{Execution Flow in Caldera}
\label{fig:execution-flow}
\end{figure}

\subsection{Implementation} \label{subsec:approach_implementation}
After describing the architecture of the Caldera framework, we will delve into the details of our attacker implementation. The attacker is deployed as a container in both the laboratory and the co-simulation. However, the terminal units presented below are only relevant for the virtual grid. In the physical setup, we rely on existing implementations from previous works, serving the purpose of checking the autonomous adaptability of the attacker.

Before detailing the attacker node implementation, we explain the modifications made to the co-simulation's terminal units. The default terminal unit runs a single process handling all the logic to be simulated, which leaves a minimal attack surface. To address this, we implemented two additional weaknesses: default passwords for remote access and vulnerability to manipulated values.

As a first vulnerability, we installed an SSH server on the terminal units. While not all manufacturers include SSH capabilities, many do, often using default settings and passwords \cite{AND16}. We set up a root user with the password `root` to exploit this vulnerability.

To simulate a supply-chain attack, we altered the script running as the main process in the terminal units to allow direct value editing during IEC 104 communication. The Python scripts for MTU and RTU were adapted to scan a predefined local folder (e.g., /tmp/upd). If a file with a specific name exists in this folder, its value overwrites the original value to be sent. This modification demonstrates how supply-chain attacks could affect smart grid components \cite{HAM23}.

The attacker was implemented as a Docker container, bundling all dependencies and configurations into one component, ensuring no need for an internet connection during execution. All dependencies are included in the attacker image during its build process, involving the installation of required packages and downloading necessary modules for Caldera.

The attacker node starts with a script initializing the C2 server, downloading the agent executable, and controlling an agent within the same container. This internal network traffic is invisible to the outside, leveraging Caldera components for further execution planning. The startup script also accepts parameters dictating the attacker's behavior, including the adversary ID, delay before launching, and timing for further instructions.

The container, run with Docker, provides full access to the host’s network, allowing the attacker to be executed similarly in both the laboratory and co-simulation.

Our attacker supports multi-stage attack emulation, dividing the attack into separate steps. Initially, the SSH brute-force adversary scans the local network, infecting vulnerable hosts. After infecting all desired victims, the second phase runs code to impact the system with some delay. The C2 server creates new operations via an API call, running specific operations on infected victims.

Executing multi-stage attacks involves respecting dependencies between attack steps. The atomic planner in Caldera ensures data collection and execution of subsequent steps as required. We explored using large language models (LLMs) to enhance attacker autonomy, but they were not reliable enough to replace Caldera's fact-based default planner.

Our implementation of attacks on terminal units targets both simulated and physical systems. The SSH brute-force attack, followed by three different attacks, demonstrates various impacts on the systems.

The SSH brute-force adversary scans the network, collects IP addresses, and uses SSH keys for authentication. It guesses login credentials from a local password list, infecting hosts by copying keys to them. Infected hosts download the agent binary from the C2 server and connect back to it, enabling lateral movement attacks.

To test confidentiality, we implemented an extraction attack, pulling sensitive data from victims. The attack extracts a list of all accessible files and their sizes, using the \texttt{du} utility, and sends this information back to the C2 server.

For integrity, we implemented a manipulation attack, tampering with IEC 104 communication. In the co-simulation, we create specific files in the /tmp/upd folder to control variable values. In the laboratory, a Python script handles value manipulation, ensuring correct communication with RTUs.

To test availability, our DoS attack renders components unavailable by disabling their network interfaces. This temporary attack ensures that physical nodes remain reachable over the network. Disabling the interface stops new commands from being sent or received, affecting communication between components.

%When deploying the attacker, key differences must be considered, such as CPU architecture variations. Raspberry Pis in the laboratory run on ARM architecture, requiring cross-compiled binaries. We used an agent implemented in Go for easy cross-compilation.

%Modular customization of attack impacts is possible by replacing operations on infected victims. Fact rules and system checks help filter IP addresses and differentiate between MTU and vRTU.

These considerations are crucial for implementing an autonomous attacker.

\subsection{Data Output}

After the scenario runs successfully, we collect data from the attacker. In the laboratory, results must be collected manually. This involves setting up packet capturing before starting components and selecting measured values on the coordinator afterward. We obtain a PCAP file with network traffic and two CSV files with transformer and load bench measurements.

In the co-simulation, this process is automated. It generates a PCAP file of traffic at the switch and CSV files with power simulation results for all desired grid components. We can define a list of components for which co-simulation exports results from Panda Power within the rettij scenario configuration. Power simulation results are exported continuously, while the network log is captured using rettij's scripting capabilities for precisely timed recordings.

The Caldera framework also exports operation results, including commands and agent responses during the attack. Logs contain details about executed abilities and host information. Similar reports can be exported after laboratory attacks, but during execution, Caldera's dashboard provides all relevant data for evaluating the attacker's performance. Automated data generation and co-simulation sequences allow us to analyze the success of individual cyberattacks after the scenarios have run.


==> chapter4.tex <==
\section{Result} \label{sec:result}
\subsection{Investigation Procedure} \label{subsec:result_proc}

To obtain reliable reference data for comparison with co-simulation results, we run cyberattacks in a laboratory using physical components to generate and balance real power loads.

The smart grid setup includes a load generator with a predefined list of loads, two inverters simulating a PV generator and a battery storage system (BSS). The PV generator has varying power output levels to mimic changing environmental conditions, while the BSS, controlled by the MTU, balances the load by either feeding energy into the grid or storing excess energy. The RTUs connected to the inverters and MTU are implemented on Raspberry Pi microcontrollers, referred to as virtual remote terminal units (vRTUs).

The RTUs, MTUs, and SCADA systems communicate via TCP/IP over Ethernet in a local area network (LAN), using protocols like IEC 104 and Modbus without additional security mechanisms. The sequence for starting scripts on vRTUs, MTU, and the coordinator is crucial for synchronized operations, leaving traces in the network logs.

Several challenges arise in this setup:
\begin{itemize}
    \item \textbf{Network Log Extraction}: Capturing all local network traffic requires a network tap. This method sometimes resulted in quadruple packet captures and inconsistent ordering, discussed further in Chapter 5.
    \item \textbf{Component Timing}: Precise timing is essential to avoid mismatches during the simulation. Any delay or failure in starting components disrupts the balance.
    \item \textbf{Warm Start}: Components are already running before the smart grid's control communication begins, making it difficult to recreate identical logging output.
\end{itemize}

This laboratory setup provides essential reference data to validate the co-simulation results, ensuring the effectiveness of our cybersecurity measures.

\subsection{Data Quality} \label{subsec:result_quality}

We assessed the quality of the generated data by analyzing different aspects of the scenarios run in the laboratory and the co-simulation. All co-simulation scenarios were run for 20 minutes, while the laboratory results varied due to manual coordination and component failures. The attacker was assumed to have gained access to the LAN via phishing or physical access. Each scenario used a zero-second wait for the attacker to start and a ten-minute delay before the second phase.

Figure 5.1 shows the measured results of the scenarios run in the physical grid. The first plot (Figure 5.1a) shows the normal behavior of the grid, serving as a reference for evaluating the impact of different cyberattacks. The grid load balances around an equilibrium at 0kW, with small peaks due to the PV system and the BSS adjusting to changes in load.

In Figure 5.1b, the DoS attack causes imbalances after ten minutes, corresponding to minute twelve in the graph. The suspended communication between the vRTU and MTU leads to significant imbalances. The PV continues to change its output independently of the MTU commands.

The extraction scenario in Figure 5.1c closely resembles the normal scenario, as the attack collects information without disrupting ongoing processes. The higher peak at the start is an example of slight differences in load balancing outcomes.

The manipulation attack in Figure 5.1d shows a huge imbalance after the second phase of the attack, similar to the DoS scenario. The BSS stops adapting to the load, causing imbalances. The PV output increases just before the end, evening out the grid load slightly.

Comparing these results to the co-simulation (Figure 5.2), the normal scenario (Figure 5.2a) shows homogeneous load balancing. The DoS attack (Figure 5.2b) results in the BSS remaining constant after the second phase, causing high imbalances. The extraction scenario (Figure 5.2c) matches the normal scenario, while the manipulation attack (Figure 5.2d) shows the BSS power level set to zero after the second phase.

The co-simulation produces consistent data (NF6), while the laboratory results showed some dissimilarities due to physical hardware noise and timing differences.

Figure 5.3 shows the protocol distributions for the laboratory scenarios. SSH traffic is the most dominant, even without an attack, due to the SSH connections needed to run scripts on the terminal units. The IEC 104 traffic fluctuates, and ARP and STP packets are common. The DoS attack reduces IEC 104 communication by half, while the extraction and manipulation scenarios show consistent IEC 104 traffic.

In the co-simulation (Figure 5.4), IEC 104 is the main protocol used. ARP packets are higher at the start, and SSH traffic is significant during attacks. The HTTP requests from infected victims are sparse.

Figure 5.5 shows the packet distribution over time in the laboratory. Without any attack, the communication baseline is around 150-200 packets per interval. The DoS attack interrupts the MTU and vRTU communication, reducing traffic. The extraction scenario shows a small increase in packets when data is sent back to the attacker. The manipulation attack blends in with ongoing communication.

In the co-simulation (Figure 5.6), traffic volume rises after five minutes due to ARP requests. The SSH brute-force attack shows regular peaks, with consistent packet distribution across intervals.

Figure 5.7 shows the traffic volume between components in the laboratory. SSH traffic dominates, with inconsistencies in data volume between scenarios. The DoS attack reduces traffic significantly, while the extraction and manipulation scenarios show consistent traffic volumes.

In the co-simulation (Figure 5.9), the IEC 104 communication is more consistent. The attacker sends large volumes of data, similar to the laboratory results.

The results demonstrate that our autonomous agent reliably generates network logs during cyberattacks on smart grids, in both physical and co-simulation environments. The attacks show similar impacts on both environments, though with some differences due to the inherent characteristics of each setup. The autonomous agent provides a systematic and consistent approach to generating data, streamlining the execution of cyberattacks.

\subsection{Application of LLMs} \label{subsec:result_llm}

As a final step in our evaluation, we investigated how well the structured representation of Caldera’s abilities and adversaries can be consumed by Large Language Models (LLMs). Combining the automated structure for running scenarios with the analytical power of LLMs could potentially enhance automation in data generation.

All abilities are defined with properties and code snippets, saved in files named after their IDs, forming a systematic information source. This modular definition includes patterns like recurring descriptions and executors, which could guide LLMs and reduce potential hallucinations.

We tested three state-of-the-art open-source LLMs pre-trained on large code bases and focused on code generation, given our hardware constraints (NVIDIA GeForce RTX 3060 Ti with 8 GB VRAM). The selected models were:

\begin{itemize}
    \item \textbf{Code Llama}: A model with 13 billion parameters, used as a reference.
    \item \textbf{DeepSeek Coder}: A 6.7 billion parameter model, reported to perform on par with larger models.
    \item \textbf{StarCoder 2}: A specialized code generation model with strong benchmark performance.
\end{itemize}

These models were tested for their ability to run on smaller hardware setups, making the results relevant for portable hardware applications.

We tested the LLMs’ understanding and generation of abilities and adversaries through four tasks: 

\begin{enumerate}
    \item \textbf{Ability Explanation}: Testing the understanding of individual abilities.
    \item \textbf{Ability Generation}: Creating a network scan in a specified format.
    \item \textbf{Adversary Explanation}: Describing the actions taken by an adversary.
    \item \textbf{Adversary Generation}: Listing abilities to form an adversary based on a described attack.
\end{enumerate}

The tests were conducted using the PrivateGPT project and ollama, with the nomic-embed-text-v1.5 embedder for effective local file reference.


Code Llama struggled with the task, providing contradictory explanations and self-generated abilities not matching the requested ID. DeepSeek Coder gave detailed explanations but referred to the wrong ability, while StarCoder 2 produced heavily hallucinated outputs.


Code Llama produced a viable solution, though with some inaccuracies. DeepSeek Coder generated code with additional unnecessary commands. StarCoder 2 failed to produce coherent output, generating hallucinated and irrelevant text.


Code Llama and DeepSeek Coder both failed to correctly explain the adversary, providing imaginary abilities and mismatched IDs. StarCoder 2 again produced incoherent output, stuck in a loop of irrelevant text.

Code Llama provided a brief and inaccurate list. DeepSeek Coder included useful properties but referenced incorrect abilities. StarCoder 2 failed to generate meaningful results, repeating irrelevant text.


These tests indicate that the selected LLMs are not well-suited for direct implementation of abilities or adversaries into Caldera. However, DeepSeek Coder showed potential for assisting in the development process by providing useful references and explanations.

Overall, while the automation of ability generation using LLMs is promising, the models tested here require further refinement and larger counterparts to achieve reliable results. Future research could explore the use of more powerful models and their integration with detailed knowledge of smart grids and protocols.



==> chapter5.tex <==
\section{Conclusion} \label{sec:conclusion}
After examining the results, let's recapitulate our work and how we met the requirements.

First, we introduced the laboratory setup for data collection. We then presented the co-simulation environment, which allowed us to develop and test our agent, satisfying requirement F1 with its power simulation and network capabilities. Using the switch component, we met requirement F2 for recordable network traffic. The attacker, implemented as a container for deployment in the co-simulation, fulfilled requirement F3. The attacker was built for offline deployment, meeting NF5.

We also configured the virtual smart grid with reusable components managed by rettij, fulfilling NF2. The automation capabilities of rettij allowed for specific scripts to run on nodes within the co-simulation, meeting NF4 for automated data output.

We deployed the attacker with our developed abilities and adversaries into the laboratory, demonstrating similar attack effects in both environments. This showed that identical attacks resulted in similar anomalies in both settings. Although the network logs did not perfectly match, the results were clean and consistent, satisfying NF6. The co-simulation results were almost perfectly reproducible, showing the impacts of attacks were transferable between the laboratory and the co-simulation, fulfilling NF1.

To ensure the security of critical infrastructure, including smart grids, further research is needed. Our framework can be applied to more complex scenarios, such as larger grid topologies resembling real-world smart grids. For example, using networks developed by the CIGRE Task Force, we can adapt our attacks to a variety of scenarios and generate corresponding network logs. Larger topologies allow for more complex connections, making lateral movement necessary to achieve goals. Our modular agent can repeat brute-force attacks on new victims, facilitating further research on complex topologies and nested attacks.

More automation is also promising. Although our results with LLMs were not as fruitful as hoped, they hold potential for automating cyberattack development in co-simulations. Using reinforcement learning, a pipeline could generate and evaluate topologies and attackers iteratively, improving both over time. Although far from the current state, further development might bring us closer to this goal.

